Navigating Complexity: Toward Lossless Graph Condensation via Expanding Window Matching

Graph condensation aims to reduce the size of a large-scale graph dataset by synthesizing a compact counterpart without sacrificing the performance of Graph Neural Networks (GNNs) trained on it, which has shed light on reducing the computational cost for training GNNs. Nevertheless, existing methods often fall short of accurately replicating the original graph for certain datasets, thereby failing to achieve the objective of lossless condensation. To understand this phenomenon, we investigate the potential reasons and reveal that the previous state-of-the-art trajectory matching method provides biased and restricted supervision signals from the original graph when optimizing the condensed one. This significantly limits both the scale and efficacy of the condensed graph. In this paper, we make the first attempt toward \textit{lossless graph condensation} by bridging the previously neglected supervision signals. Specifically, we employ a curriculum learning strategy to train expert trajectories with more diverse supervision signals from the original graph, and then effectively transfer the information into the condensed graph with expanding window matching. Moreover, we design a loss function to further extract knowledge from the expert trajectories. Theoretical analysis justifies the design of our method and extensive experiments verify its superiority across different datasets. Code is released at https://github.com/NUS-HPC-AI-Lab/GEOM.

==> Table/cross_.tex <==
% \usepackage{array} % for \extrarowheight
% \setlength{\extrarowheight}{8pt}
\definecolor{highlightcolor}{RGB}{198, 239, 252}  % 设置为你想要的颜色
\sethlcolor{highlightcolor}

\begin{table*}[ht]
\centering
\tiny
% \renewcommand\arraystretch{1.1} 
\renewcommand\arraystretch{0.8}
\setlength{\extrarowheight}{1.5pt} % 调整行高
% \small % 使用\small来设置表格内文本的字体大小为小号
\caption{Performance across different GNN architectures. \colorbox{orange!30}{\makebox(14,6){Avg.}} and \colorbox{red!30}{\makebox(15,6){Std.}}: the average performance and the standard deviation of the results of all architectures, \colorbox{cyan!20}{\makebox(20,6){$\Delta$(\%)}} denotes the improvements upon the DC-Graph. \colorbox{gray!20}{GCN} indicates that the synthetic graph is condensed with GCN. \textbf{Bold entries} are best results, \underline{underline} marks the lossless results.}
\label{tab:cross}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{cccccccccccccc}
% {|l| >{\columncolor{gray!40}} l|l|}
\cline{1-12}
                          &         & \multicolumn{7}{c}{Architectures}                & \multicolumn{3}{c}{Statistics}                                                                                          \\ \cline{3-12}
                          % \cellcolor{gray!40}
\multirow{-2}{*}{Datasets} & \multirow{-2}{*}{Methods} & MLP  & GAT  & APPNP & Cheby & \cellcolor{gray!40}GCN & SAGE & SGC & \cellcolor[HTML]{FFE6CC}Avg.          & \cellcolor[HTML]{FFB2B2}Std.          & \cellcolor[HTML]{C6EFFC}$\Delta$(\%)  \\ \cline{1-9}


                                                      & DC-Graph & 66.2 & - &66.4 &64.9 &\cellcolor{gray!40}66.2 &65.9 &69.6 &  \cellcolor[HTML]{FFE6CC}66.5          & \cellcolor[HTML]{FFB2B2}1.5         & \cellcolor[HTML]{C6EFFC}-               \\


                          & GCond & 63.9 &55.4 &69.6 &68.3 &\cellcolor{gray!40}70.5 &66.2 &70.3 & \cellcolor[HTML]{FFE6CC}66.3         & \cellcolor[HTML]{FFB2B2}5.0         & $\downarrow$ \cellcolor[HTML]{C6EFFC}0.2       \\
                           & SFGC & 71.3 & 72.1 &70.5 &71.8& \cellcolor{gray!40}71.6 &71.7& 71.8&  \cellcolor[HTML]{FFE6CC}71.5          & \cellcolor[HTML]{FFB2B2}0.5          & $\uparrow$ \cellcolor[HTML]{C6EFFC}5.0         \\

\multirow{-5}{*}{\centering Citeseer}
& GEOM & 74.2 & 74.2 & 74.0 & 74.1  &\cellcolor{gray!40}74.3 & 74.1 & 74.3 & \cellcolor[HTML]{FFE6CC}\textbf{74.2} & \cellcolor[HTML]{FFB2B2}0.1 & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{7.7}   \\ \cline{1-9}
\multirow{-5}{*}{\centering ($r$ = 1.80\%)}

                                                          & DC-Graph & 67.2 & - &67.1 &67.7 &\cellcolor{gray!40}67.9 &66.2 &72.8 &  \cellcolor[HTML]{FFE6CC}68.1          & \cellcolor[HTML]{FFB2B2}2.1          & \cellcolor[HTML]{C6EFFC}-               \\

                          & GCond & 73.1 &66.2 &78.5 &76.0 &\cellcolor{gray!40}80.1 &78.2 &79.3 & \cellcolor[HTML]{FFE6CC}75.9          & \cellcolor[HTML]{FFB2B2}4.5         &  $\uparrow$ \cellcolor[HTML]{C6EFFC}7.8         \\
                           & SFGC & 81.1& 80.8 &78.8 &79.0& \cellcolor{gray!40}81.1 &81.9& 79.1&  \cellcolor[HTML]{FFE6CC}80.3         & \cellcolor[HTML]{FFB2B2}1.2          & $\uparrow$ \cellcolor[HTML]{C6EFFC}12.2            \\

\multirow{-5}{*}{Cora}  & GEOM & 83.6 & 82.7 & 82.8 & 80.7  &\cellcolor{gray!40}83.6 & 83.7 & 83.1 & \cellcolor[HTML]{FFE6CC}\textbf{82.9} & \cellcolor[HTML]{FFB2B2}1.0 & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{14.8}  \\ \cline{1-9}
\multirow{-5}{*}{\centering ($r$ = 2.60\%)}
                          & DC-Graph & 59.9& -& 60.0& 55.7 &\cellcolor{gray!40}59.8 &60.0 & 60.4 & \cellcolor[HTML]{FFE6CC}59.3          & \cellcolor[HTML]{FFB2B2}1.6           & \cellcolor[HTML]{C6EFFC}-               \\

                          & GCond & 62.2& 60.0 &63.4 &54.9& \cellcolor{gray!40}63.2 &62.6& 63.7&  \cellcolor[HTML]{FFE6CC}61.4          & \cellcolor[HTML]{FFB2B2}2.9          &  $\uparrow$ \cellcolor[HTML]{C6EFFC}2.1              \\
                           & SFGC & 65.1& 65.7 &63.9 &60.7& \cellcolor{gray!40}65.1 &64.8& 64.8&  \cellcolor[HTML]{FFE6CC}64.3          & \cellcolor[HTML]{FFB2B2}1.6         & $\uparrow$ \cellcolor[HTML]{C6EFFC}5.0             \\
           
\multirow{-5}{*}{Ogbn-arxiv}   & GEOM & 68.8 & 66.4 &65.8 & 62.5 &\cellcolor{gray!40}68.8 & 68.9 & 66.4  & \cellcolor[HTML]{FFE6CC}\textbf{66.8} & \cellcolor[HTML]{FFB2B2}2.1  & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{7.5}   \\ \cline{1-9}
\multirow{-5}{*}{\centering ($r$ = 0.25\%)}





                          & DC-Graph &43.1 & -& 45.7 &43.8 &\cellcolor{gray!40}45.9 &45.8 &45.6  & \cellcolor[HTML]{FFE6CC}45.0        & \cellcolor[HTML]{FFB2B2}1.1         & \cellcolor[HTML]{C6EFFC}-           \\
                           & GCond & 44.8 & 40.1 & 45.9 & 42.8 & \cellcolor{gray!40}47.1& 46.2& 46.1 & \cellcolor[HTML]{FFE6CC}44.7         & \cellcolor[HTML]{FFB2B2}2.3           & $\downarrow$ \cellcolor[HTML]{C6EFFC}0.3              \\
                           & SFGC & 47.1 & 45.3 & 40.7 & 45.4 &\cellcolor{gray!40}47.1& 47.0& 42.5 & \cellcolor[HTML]{FFE6CC}45.0        & \cellcolor[HTML]{FFB2B2}2.3           & \cellcolor[HTML]{C6EFFC}-             \\
\multirow{-5}{*}{Flickr}     & GEOM & 47.0 & 42.1 & 46.6 & 45.3 & \cellcolor{gray!40}47.3 &47.1 &46.3 & \cellcolor[HTML]{FFE6CC}\textbf{46.0} & \cellcolor[HTML]{FFB2B2}1.7  & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{1.0}   \\ \cline{1-9}
\multirow{-5}{*}{\centering ($r$ = 0.50\%)}
                           & DC-Graph & 50.3 & - & 81.2 & 77.5 & \cellcolor{gray!40}89.5 & 89.7 & 90.5 & \cellcolor[HTML]{FFE6CC}79.8         & \cellcolor[HTML]{FFB2B2}14.0          & \cellcolor[HTML]{C6EFFC}-              \\
                           & GCond & 42.5 & 60.2 & 87.8 & 75.5 & \cellcolor{gray!40}89.4 & 89.1 & 89.6 & \cellcolor[HTML]{FFE6CC}76.3          & \cellcolor[HTML]{FFB2B2}17.1          &  $\downarrow$ \cellcolor[HTML]{C6EFFC}3.5             \\
                          & SFGC & 89.5 & 87.1 & 88.3 & 82.8 & \cellcolor{gray!40}89.7 & 90.3 & 89.5 & \cellcolor[HTML]{FFE6CC}88.2          & \cellcolor[HTML]{FFB2B2}2.4           & $\uparrow$ \cellcolor[HTML]{C6EFFC}8.4             \\
\multirow{-5}{*}{Reddit} & GEOM & 91.4 & 90.0 & 87.9 & 82.7 & \cellcolor{gray!40}91.4 & 91.4 & 89.3 & \cellcolor[HTML]{FFE6CC}\textbf{89.2}  & \cellcolor[HTML]{FFB2B2}2.9  & \cellcolor[HTML]{C6EFFC}$\uparrow$ \textbf{9.4}  \\ \cline{1-12}
\multirow{-5}{*}{\centering ($r$ = 0.10\%)}

                           & DC-Graph & 61.2 & - &61.4 &58.3& \cellcolor{gray!40}61.1 &60.9& 61.3&  \cellcolor[HTML]{FFE6CC}60.7          & \cellcolor[HTML]{FFB2B2}1.1         &  \cellcolor[HTML]{C6EFFC}-             \\
                           & SFGC & 69.4& 69.6 &68.7 &64.7& \cellcolor{gray!40}69.4 &69.4& 69.1&  \cellcolor[HTML]{FFE6CC}68.5          & \cellcolor[HTML]{FFB2B2}1.6         &  \cellcolor[HTML]{C6EFFC}$\uparrow$7.8            \\
           
\multirow{-3.7}{*}{Ogbn-arxiv}   & GEOM & 71.2 & 70.0 &69.1 & 64.5 &\cellcolor{gray!40}71.4 & 71.1 & 69.6  & \cellcolor[HTML]{FFE6CC}\textbf{69.6} & \cellcolor[HTML]{FFB2B2}2.2  & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{8.9}   \\ \cline{1-9}
\multirow{-3.5}{*}{\centering ($r$ = 5.00\%)}

                           & DC-Graph & 52.3 & - &84.1 &81.2& \cellcolor{gray!40}90.3 &90.6& 90.9&  \cellcolor[HTML]{FFE6CC}81.6          & \cellcolor[HTML]{FFB2B2}13.6         &  \cellcolor[HTML]{C6EFFC}-             \\


                           & SFGC & 91.6 & 90.3 &91.1 &85.3& \cellcolor{gray!40}91.9 &91.6& 90.9&  \cellcolor[HTML]{FFE6CC}90.4          & \cellcolor[HTML]{FFB2B2}2.1         &  \cellcolor[HTML]{C6EFFC}$\uparrow$8.8             \\
\multirow{-3.7}{*}{Reddit} & GEOM & 93.9 & 93.0 & 92.4 & 88.5 & \cellcolor{gray!40}93.9 & 93.8 & 92.7 & \cellcolor[HTML]{FFE6CC}\textbf{92.6}  & \cellcolor[HTML]{FFB2B2}1.8  & \cellcolor[HTML]{C6EFFC}$\uparrow$ \textbf{11.0}   \\ \cline{1-12}
\multirow{-3.5}{*}{\centering ($r$ = 5.00\%)}
                          % &         &      &      &       &       &      &      &      &                                       &                                       &                                       &  & 
\end{tabular}%
}
\vspace{-2.5em}
\end{table*}

==> Table/cross_re.tex <==
% \usepackage{array} % for \extrarowheight
% \setlength{\extrarowheight}{8pt}
\definecolor{highlightcolor}{RGB}{198, 239, 252}  % 设置为你想要的颜色
\sethlcolor{highlightcolor}

\begin{table*}[ht]
\centering
\tiny
% \renewcommand\arraystretch{1.1} 
\renewcommand\arraystretch{0.8}
\setlength{\extrarowheight}{1.5pt} % 调整行高
% \small % 使用\small来设置表格内文本的字体大小为小号
\caption{Performance across different GNN architectures. \colorbox{orange!30}{\makebox(14,6){Avg.}} and \colorbox{red!30}{\makebox(15,6){Std.}}: the average performance and the standard deviation of the results of all architectures, \colorbox{cyan!20}{\makebox(20,6){$\Delta$(\%)}} denotes the improvements upon the DC-Graph. \colorbox{gray!20}{GCN} indicates that the synthetic graph is condensed with GCN. \textbf{Bold entries} are best results, \underline{underline} marks the lossless results.}
\label{tab:cross}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{cccccccccccccc}
% {|l| >{\columncolor{gray!40}} l|l|}
\cline{1-12}
                          &         & \multicolumn{7}{c}{Architectures}                & \multicolumn{3}{c}{Statistics}                                                                                          \\ \cline{3-12}
                          % \cellcolor{gray!40}
\multirow{-2}{*}{Datasets} & \multirow{-2}{*}{Methods} & MLP  & GAT  & APPNP & Cheby & \cellcolor{gray!40}GCN & SAGE & SGC & \cellcolor[HTML]{FFE6CC}Avg.          & \cellcolor[HTML]{FFB2B2}Std.          & \cellcolor[HTML]{C6EFFC}$\Delta$(\%)  \\ \cline{1-9}


                                                      & DC-Graph & 66.2 & - &66.4 &64.9 &\cellcolor{gray!40}66.2 &65.9 &69.6 &  \cellcolor[HTML]{FFE6CC}66.5          & \cellcolor[HTML]{FFB2B2}1.5         & \cellcolor[HTML]{C6EFFC}-               \\


                          & GCond & 63.9 &55.4 &69.6 &68.3 &\cellcolor{gray!40}70.5 &66.2 &70.3 & \cellcolor[HTML]{FFE6CC}66.3         & \cellcolor[HTML]{FFB2B2}5.0         & $\downarrow$ \cellcolor[HTML]{C6EFFC}0.2       \\
                           & SFGC &\underline{71.3} & \underline{72.1} &70.5 &\underline{71.8}& \cellcolor{gray!40}71.6 &\underline{71.7}& \underline{71.8}&  \cellcolor[HTML]{FFE6CC}71.5          & \cellcolor[HTML]{FFB2B2}0.5          & $\uparrow$ \cellcolor[HTML]{C6EFFC}5.0         \\

\multirow{-5}{*}{\centering Citeseer}
& GEOM & \underline{74.2} & \underline{74.2} & \underline{74.0} & \underline{74.1}  &\cellcolor{gray!40}\underline{74.3} & \underline{74.1} & \underline{74.3} & \cellcolor[HTML]{FFE6CC}\textbf{74.2} & \cellcolor[HTML]{FFB2B2}0.1 & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{7.7}   \\ \cline{1-9}
\multirow{-5}{*}{\centering ($r$ = 1.80\%)}

                                                          & DC-Graph & 67.2 & - &67.1 &67.7 &\cellcolor{gray!40}67.9 &66.2 &72.8 &  \cellcolor[HTML]{FFE6CC}68.1          & \cellcolor[HTML]{FFB2B2}2.1          & \cellcolor[HTML]{C6EFFC}-               \\

                          & GCond & 73.1 &66.2 &78.5 &76.0 &\cellcolor{gray!40}80.1 &78.2 &79.3 & \cellcolor[HTML]{FFE6CC}75.9          & \cellcolor[HTML]{FFB2B2}4.5         &  $\uparrow$ \cellcolor[HTML]{C6EFFC}7.8         \\
                           & SFGC & \underline{81.1}& 80.8 &78.8 &79.0& \cellcolor{gray!40}81.1 &\underline{81.9}& 79.1&  \cellcolor[HTML]{FFE6CC}80.3         & \cellcolor[HTML]{FFB2B2}1.2          & $\uparrow$ \cellcolor[HTML]{C6EFFC}12.2            \\

\multirow{-5}{*}{Cora}  & GEOM & \underline{83.6} & 82.7 & 82.8 & 80.7  &\cellcolor{gray!40}\underline{83.6} & \underline{83.7} & \underline{83.1} & \cellcolor[HTML]{FFE6CC}\textbf{82.9} & \cellcolor[HTML]{FFB2B2}1.0 & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{14.8}  \\ \cline{1-9}
\multirow{-5}{*}{\centering ($r$ = 2.60\%)}
                          & DC-Graph & 59.9& -& 60.0& 55.7 &\cellcolor{gray!40}59.8 &60.0 & 60.4 & \cellcolor[HTML]{FFE6CC}59.3          & \cellcolor[HTML]{FFB2B2}1.6           & \cellcolor[HTML]{C6EFFC}-               \\

                          & GCond & 62.2& 60.0 &63.4 &54.9& \cellcolor{gray!40}63.2 &62.6& 63.7&  \cellcolor[HTML]{FFE6CC}61.4          & \cellcolor[HTML]{FFB2B2}2.9          &  $\uparrow$ \cellcolor[HTML]{C6EFFC}2.1              \\
                           & SFGC & 65.1& 65.7 &63.9 &60.7& \cellcolor{gray!40}65.1 &64.8& 64.8&  \cellcolor[HTML]{FFE6CC}64.3          & \cellcolor[HTML]{FFB2B2}1.6         & $\uparrow$ \cellcolor[HTML]{C6EFFC}5.0             \\
           
\multirow{-5}{*}{Ogbn-arxiv}   & GEOM & \underline{68.8} & 66.4 &65.8 & 62.5 &\cellcolor{gray!40}68.8 & 68.9 & 66.4  & \cellcolor[HTML]{FFE6CC}\textbf{66.8} & \cellcolor[HTML]{FFB2B2}2.1  & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{7.5}   \\ \cline{1-9}
\multirow{-5}{*}{\centering ($r$ = 0.25\%)}

                           & DC-Graph & 61.2 & - &61.4 &58.3& \cellcolor{gray!40}61.1 &60.9& 61.3&  \cellcolor[HTML]{FFE6CC}60.7          & \cellcolor[HTML]{FFB2B2}1.1         &  \cellcolor[HTML]{C6EFFC}-             \\
                           & SFGC & \underline{69.4}& 69.6 &68.7 &64.7& \cellcolor{gray!40}69.4 &69.4& 69.1&  \cellcolor[HTML]{FFE6CC}68.5          & \cellcolor[HTML]{FFB2B2}1.6         &  \cellcolor[HTML]{C6EFFC}$\uparrow$7.8            \\
           
\multirow{-3.7}{*}{Ogbn-arxiv}   & GEOM & \underline{71.2} & 70.0 &69.1 & 64.5 &\cellcolor{gray!40}\underline{71.4} & 71.1 & 69.6  & \cellcolor[HTML]{FFE6CC}\textbf{69.6} & \cellcolor[HTML]{FFB2B2}2.2  & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{8.9}   \\ \cline{1-9}
\multirow{-3.5}{*}{\centering ($r$ = 5.00\%)}



                          & DC-Graph &43.1 & -& 45.7 &43.8 &\cellcolor{gray!40}45.9 &45.8 &45.6  & \cellcolor[HTML]{FFE6CC}45.0        & \cellcolor[HTML]{FFB2B2}1.1         & \cellcolor[HTML]{C6EFFC}-           \\
                           & GCond & 44.8 & 40.1 & 45.9 & 42.8 & \cellcolor{gray!40}47.1& 46.2& 46.1 & \cellcolor[HTML]{FFE6CC}44.7         & \cellcolor[HTML]{FFB2B2}2.3           & $\downarrow$ \cellcolor[HTML]{C6EFFC}0.3              \\
                           & SFGC & 47.1 & \underline{45.3} & 40.7 & 45.4 &\cellcolor{gray!40}47.1& \underline{47.0}& 42.5 & \cellcolor[HTML]{FFE6CC}45.0        & \cellcolor[HTML]{FFB2B2}2.3           & \cellcolor[HTML]{C6EFFC}-             \\
\multirow{-5}{*}{Flickr}     & GEOM & 47.0 & 42.1 & 46.6 & 45.3 & \cellcolor{gray!40}\underline{47.3} &\underline{47.1} &\underline{46.3} & \cellcolor[HTML]{FFE6CC}\textbf{46.0} & \cellcolor[HTML]{FFB2B2}1.7  & $\uparrow$ \cellcolor[HTML]{C6EFFC}\textbf{1.0}   \\ \cline{1-9}
\multirow{-5}{*}{\centering ($r$ = 0.50\%)}
                           & DC-Graph & 50.3 & - & 81.2 & 77.5 & \cellcolor{gray!40}89.5 & 89.7 & 90.5 & \cellcolor[HTML]{FFE6CC}79.8         & \cellcolor[HTML]{FFB2B2}14.0          & \cellcolor[HTML]{C6EFFC}-              \\
                           & GCond & 42.5 & 60.2 & 87.8 & 75.5 & \cellcolor{gray!40}89.4 & 89.1 & 89.6 & \cellcolor[HTML]{FFE6CC}76.3          & \cellcolor[HTML]{FFB2B2}17.1          &  $\downarrow$ \cellcolor[HTML]{C6EFFC}3.5             \\
                          & SFGC & 89.5 & 87.1 & 88.3 & 82.8 & \cellcolor{gray!40}89.7 & 90.3 & 89.5 & \cellcolor[HTML]{FFE6CC}88.2          & \cellcolor[HTML]{FFB2B2}2.4           & $\uparrow$ \cellcolor[HTML]{C6EFFC}8.4             \\
\multirow{-5}{*}{Reddit} & GEOM & 91.4 & 90.0 & 87.9 & 82.7 & \cellcolor{gray!40}91.4 & 91.4 & 89.3 & \cellcolor[HTML]{FFE6CC}\textbf{89.2}  & \cellcolor[HTML]{FFB2B2}2.9  & \cellcolor[HTML]{C6EFFC}$\uparrow$ \textbf{9.4}  \\ \cline{1-12}
\multirow{-5}{*}{\centering ($r$ = 0.10\%)}



                           & DC-Graph & 52.3 & - &84.1 &81.2& \cellcolor{gray!40}90.3 &90.6& 90.9&  \cellcolor[HTML]{FFE6CC}81.6          & \cellcolor[HTML]{FFB2B2}13.6         &  \cellcolor[HTML]{C6EFFC}-             \\


                           & SFGC & 91.6 & 90.3 &91.1 &85.3& \cellcolor{gray!40}91.9 &91.6& 90.9&  \cellcolor[HTML]{FFE6CC}90.4          & \cellcolor[HTML]{FFB2B2}2.1         &  \cellcolor[HTML]{C6EFFC}$\uparrow$8.8             \\
\multirow{-3.7}{*}{Reddit} & GEOM & \underline{93.9} & \underline{93.0} & 92.4 & 88.5 & \cellcolor{gray!40}\underline{93.9} & \underline{93.8} & 92.7 & \cellcolor[HTML]{FFE6CC}\textbf{92.6}  & \cellcolor[HTML]{FFB2B2}1.8  & \cellcolor[HTML]{C6EFFC}$\uparrow$ \textbf{11.0}   \\ \cline{1-12}
\multirow{-3.5}{*}{\centering ($r$ = 5.00\%)}
                          % &         &      &      &       &       &      &      &      &                                       &                                       &                                       &  & 
\end{tabular}%
}
\vspace{-2.5em}
\end{table*}

==> Table/nc.tex <==

\definecolor{lightblue}{RGB}{1,216,230}
\sethlcolor{lightblue}

\begin{table*}[ht]
  \centering
  \caption{Performance comparison to baselines in the node classification tasks. \textit{the highest results in most cases
  on node classification and lossless results on all datasets.} We report test accuracy (\%) on Citeseer, Cora, Ogbn-arxiv, Flickr and Reddit. \textbf{Bold entries} are best results, \hl{highlight} marks the lossless results. The structure optimization component of GCOND can be used to optimize larger composite diagrams out of memory (oom).}
  \label{tab:nc}
  \scriptsize
   \begin{tabular}{cc|ccccccc|c|c}
   % \begin{tabular}{cc|cccc|ccc|c|c}
    \toprule
    Dataset & Ratio & Random & Herding & K-Center & DC-Graph & GCond & GCond-X & SFGC & (ours) & Whole Dataset\\
    \midrule
    \multirow{3}{*}{Citeseer} & 0.90\% & 54.4$_{\pm 4.4}$ & 57.1$_{\pm 1.5}$ & 52.4$_{\pm 2.8}$ & 66.8$_{\pm 1.5}$ & 70.5$_{\pm 1.2}$ & 71.4$_{\pm 0.8}$ & \underline{71.4$_{\pm 0.5}$} & 
    
    \textbf{\hl{73.0$_{\pm 0.5}$}} & \multirow{3}{*}{71.7$_{\pm 0.1}$} \\
    & 1.80\% & 64.2$_{\pm 1.7}$ & 66.7$_{\pm 1.0}$ & 64.3$_{\pm 1.0}$ &  59.0$_{\pm 0.5}$ & 70.6$_{\pm 0.9}$ & 69.8$_{\pm 1.1}$ & \underline{\hl{72.4$_{\pm 0.4}$}} & 
    
    \textbf{\hl{74.3$_{\pm 0.1}$}} \\
     & 3.60\% & 69.1$_{\pm 0.1}$ & 69.0$_{\pm 0.1}$ & 69.1$_{\pm 0.1}$ & 66.3$_{\pm 1.5}$  & 69.8$_{\pm 1.4}$ & 69.4$_{\pm 1.4}$ & \underline{70.6$_{\pm 0.7}$} & 
     
     \textbf{\hl{73.3$_{\pm 0.4}$}} \\
    \midrule
    \multirow{3}{*}{Cora} & 1.30\%  & 63.6$_{\pm 3.7}$ & 67.0$_{\pm 1.3}$ & 64.0$_{\pm 2.3}$ & 67.3$_{\pm 1.9}$ &  79.8$_{\pm 1.3}$ & 75.9$_{\pm 1.2}$ & \underline{80.1$_{\pm 0.4}$} & 
    
    \textbf{\hl{82.5$_{\pm 0.4}$}} & \multirow{3}{*}{81.2$_{\pm 0.2}$} \\
    & 2.60\% &72.8$_{\pm 1.1}$ & 73.4$_{\pm 1.0}$ & 73.2$_{\pm 1.2}$  & 67.6$_{\pm 3.5}$ &  80.1$_{\pm 0.6}$ & 75.7$_{\pm 0.9}$ & \underline{\hl{81.7$_{\pm 0.5}$}} & 
    
    \textbf{\hl{83.6$_{\pm 0.3}$}} \\
     & 5.20\%  & 76.8$_{\pm 0.1}$ & 76.8$_{\pm 0.1}$ & 76.7$_{\pm 0.1}$ & 67.7$_{\pm 2.2}$ & 79.3$_{\pm 0.3}$ & 76.0$_{\pm 0.3}$ & \underline{\hl{81.6$_{\pm 0.8}$}} & 
     
     \textbf{\hl{82.8$_{\pm 0.7}$}} \\
    \midrule
    \multirow{5}{*}{Ogbn-arxiv} & 0.05\% & 47.1$_{\pm 3.9}$ & 52.4$_{\pm 1.8}$ & 47.2$_{\pm 3.0}$ & 58.6$_{\pm 0.4}$ & 59.2$_{\pm 1.1}$ & 61.3$_{\pm 0.5}$ & \underline{65.5$_{\pm 0.7}$} & 
    \textbf{65.5$_{\pm 0.6}$} & \multirow{5}{*}{71.4$_{\pm 0.1}$} \\
    
    & 0.25\%  &57.3$_{\pm 1.1}$ & 58.6$_{\pm 1.2}$ & 56.8$_{\pm 0.8}$ & 59.9$_{\pm 0.3}$ &63.2$_{\pm 0.3}$ & 64.2$_{\pm 0.4}$ & \underline{66.1$_{\pm 0.4}$} & 
    \textbf{68.8$_{\pm 0.2}$} \\
    
     & 0.50\%  &60.0$_{\pm 0.9}$ & 60.4$_{\pm 0.8}$ & 60.3$_{\pm 0.4}$ & 59.5$_{\pm 0.3}$ &  64.0$_{\pm 1.4}$ & 63.1$_{\pm 0.5}$ & \underline{66.8$_{\pm 0.4}$} & 
     \textbf{69.6$_{\pm 0.2}$} \\

    & 2.50\%  &64.1$_{\pm 0.7}$ & 64.3$_{\pm 0.8}$ & 64.1$_{\pm 0.5}$ & 61.3$_{\pm 0.3}$ &  66.3$_{\pm 1.1}$ & 66.1$_{\pm 0.3}$ & \underline{68.3$_{\pm 0.3}$} & 
     \textbf{71.0$_{\pm 0.1}$} \\

    & 5.00\%  &66.0$_{\pm 0.6}$ & 66.1$_{\pm 0.4}$ & 66.2$_{\pm 0.3}$ & 66.7$_{\pm 0.3}$ &  OOM* & 66.9$_{\pm 0.4}$ & \underline{69.4$_{\pm 0.3}$} & 
     \textbf{\hl{71.4$_{\pm 0.1}$}} \\
     
      \midrule
    \multirow{3}{*}{Flickr} & 0.10\% &41.8$_{\pm 2.0}$ & 42.5$_{\pm 1.8}$ & 42.0$_{\pm 0.7}$  & 46.3$_{\pm 0.2}$ & 46.5$_{\pm 0.4}$ & 45.9$_{\pm 0.1}$ & \underline{46.6$_{\pm 0.2}$} & 
    
    \textbf{47.1$_{\pm 0.1}$} & \multirow{3}{*}{47.2$_{\pm 0.1}$} \\
    & 0.50\%  & 44.0$_{\pm 0.4}$ & 43.9$_{\pm 0.9}$ & 43.2$_{\pm 0.1}$ & 45.9$_{\pm 0.1}$ &  \textbf{47.1$_{\pm 0.1}$} & 45.0$_{\pm 0.2}$ & \underline{47.0$_{\pm 0.1}$} & 
    
    47.0$_{\pm 0.2}$ \\
     & 1.0\% & 44.6$_{\pm 0.2}$ & 44.4$_{\pm 0.6}$ & 44.1$_{\pm 0.4}$ & 44.6$_{\pm 0.1}$ &  \underline{47.1$_{\pm 0.1}$} & 45.0$_{\pm 0.2}$ & \underline{47.1$_{\pm 0.1}$} & 
     
     \textbf{\hl{47.3$_{\pm 0.3}$}} \\
      \midrule

    \multirow{5}{*}{Reddit} & 0.01\%  &46.1$_{\pm 4.4}$ & 53.1$_{\pm 2.5}$ & 46.6$_{\pm 2.3}$ & 88.2$_{\pm 0.2}$ & 88.0$_{\pm 1.8}$ & 88.4$_{\pm 0.4}$ & 
    
    \underline{89.7$_{\pm 0.2}$} & \textbf{91.1$_{\pm 0.4}$} \\
    & 0.05\% &58.0$_{\pm 2.2}$ & 62.7$_{\pm 1.0}$ & 53.0$_{\pm 3.3}$  & 89.5$_{\pm 0.1}$ &  89.6$_{\pm 0.7}$ & 89.3$_{\pm 0.1}$ & \underline{90.0$_{\pm 0.3}$} & 
    
    \textbf{91.4$_{\pm 0.2}$} &\multirow{3}{*}{93.9$_{\pm 0.0}$}\\
     & 0.50\%  &66.3$_{\pm 1.9}$ & 71.0$_{\pm 1.6}$ & 58.5$_{\pm 2.1}$ & 90.5$_{\pm 1.2}$ &  90.1$_{\pm 0.5}$ & 88.8$_{\pm 0.4}$  & \underline{90.3$_{\pm 0.3}$} & 
     
     \textbf{91.5$_{\pm 0.4}$} \\

     & 3.00\%  &73.4$_{\pm 1.3}$ & 79.3$_{\pm 1.1}$ & 71.2$_{\pm 1.4}$ & 90.8$_{\pm 0.9}$ &  OOM* & 89.2$_{\pm 0.2}$  & \underline{91.0$_{\pm 0.3}$} & 
     
     \textbf{93.7$_{\pm 0.1}$} \\


          & 5.00\%  &79.6$_{\pm 1.1}$ & 82.1$_{\pm 0.8}$ & 80.3$_{\pm 1.2}$ & 91.5$_{\pm 0.7}$ &  OOM* & 88.9$_{\pm 0.3}$  & \underline{91.9$_{\pm 0.2}$} & 
     
     \textbf{\colorbox{yellow}{93.9$_{\pm 0.1}$}} \\

     
    \bottomrule
    \end{tabular}%
  % \label{tab:performance of node classfication}%
\end{table*}
